Distributional Uncertainty Propagation via Optimal Transport

This paper addresses the limitations of standard uncertainty models, e.g., robust (norm-bounded) and stochastic (one fixed distribution, e.g., Gaussian), and proposes to model uncertainty via Optimal Transport (OT) ambiguity sets. These constitute a very rich uncertainty model, which enjoys many desirable geometrical, statistical, and computational properties, and which: (1) naturally generalizes both robust and stochastic models, and (2) captures many additional real-world uncertainty phenomena (e.g., black swan events). Our contributions show that OT ambiguity sets are also analytically tractable: they propagate easily and intuitively through linear and nonlinear (possibly corrupted by noise) transformations, and the result of the propagation is again an OT ambiguity set or can be tightly upper bounded by an OT ambiguity set. In the context of dynamical systems, our results allow us to consider multiple sources of uncertainty (e.g., initial condition, additive noise, multiplicative noise) and to capture in closed-form, via an OT ambiguity set, the resulting uncertainty in the state at any future time. Our results are actionable, interpretable, and readily employable in a great variety of computationally tractable control and estimation formulations. To highlight this, we study three applications in trajectory planning, consensus algorithms, and least squares estimation. We conclude the paper with a list of exciting open problems enabled by our results.

==> old/applications_old.tex <==
In this section, we present several applications.
In~\cref{sec:app:dynamical}, we leverage our tools to propagate distributional uncertainty through dynamical systems. We then use these results, in~\cref{sec:application:trajectory:planning,sec:application:consensus}, for distributionally robust trajectory planning and for uncertainty quantification of the consensus state of discrete-time averaging algorithms. 
Finally, in~\cref{sec:LS}, we deploy our tools to capture the distributional uncertainty of the error for the least squares estimator. 

\subsection{Dynamical Systems and Control Theory}\label{sec:app:dynamical}
Our first application concerns the propagation of the distributional uncertainty through a dynamical system. To start, consider the deterministic dynamical system
\begin{align}
\label{eq:nonlinear:dyn:sys}
    x_{t+1} = f(x_t), \quad x_0 \sim \Q_0 \in \ball{\varepsilon}{c}{\P},
\end{align}
with $f:\reals^n \to \reals^n$. %The notation $x^+$ stands for either discrete-time, in which case \eqref{eq:nonlinear:dyn:sys} is a difference equation, i.e. $x_{t+1} = f(x_t)$, or continuous-time, in which case \eqref{eq:nonlinear:dyn:sys} is an ordinary differential equation, i.e. $\dot{x} = f(x)$. 
%We denote by $\Phi_t(x_0)$ the solution map of the dynamical system \eqref{eq:nonlinear:dyn:sys} at time $t$, parametrized by the initial condition $x_0$.
%Later in this section, we will also consider the case of stochastic dynamical systems.
The initial condition $x_0$ is distributed according to some unknown probability distribution $\Q_0$, which is however known to belong to the ambiguity set $\ball{\varepsilon}{c_d}{\P}$ with center $\P\in\probSpace{\reals^d}$. This formulation encompasses the scenario when one only has access to $n$ i.i.d. samples $\{(\sample{x_0}{i})\}_{i=1}^n$ from $\Q_0$. In this case, the concentration inequality of~\cref{prop:conc:ineq} can be used to construct an \gls{acr:ot} ambiguity set $\ball{\varepsilon}{c}{\empiricalP{n}}$ around the empirical distribution $\empiricalP{n} = \frac{1}{n}\sum_{i=1}^n \diracDelta{\sample{x_0}{i}}$ which contains the true distribution $\P$ with high probability.

We now study how the distributional uncertainty encapsulated in the \gls{acr:ot} ambiguity set $\ball{\varepsilon}{c_d}{\P}$ propagates through the dynamics. This way, we can characterize the distributional uncertainty of $x_t$, which enables, among others, distributionally robust analysis and decision-making; see~\cref{sec:application:trajectory:planning} on distributionally robust trajectory planning below for an example. 
Since~\eqref{eq:nonlinear:dyn:sys} is effectively a pushforward via $f\circ\ldots\circ f$ of $\Q_0$, the result follows directly from~\cref{thm:nonlin:trans,thm:lin:trans}:

\begin{comment}
\begin{remark}\label{remark:shortcomingspropagation}
Whenever the initial distribution $\Q_0$ is known and absolutely continuous with density $\rho_0$, i.e. $\Q_0=\rho_0\lebesgueMeasure{d}$, and the transformation $f$ is a diffeomorphism,~\eqref{eq:propagation:abs:cont:distrib} can be used to recover the distribution of $\Phi_t(x_0)$ as
\begin{align*}
    \Phi_t(x_0) \sim \Q_t = \frac{\rho\circ f^{-t}}{|\det\nabla (f^t)|}\lebesgueMeasure{d}.
\end{align*}
However, in most applications, the distribution $\Q_0$ is generally unknown. Instead, it is very common to have some partial knowledge about $\Q_0$, such as some information about its first $p$ moments. Nonetheless, moments do not naturally propagate through the nonlinear dynamics. Indeed, let $\Q$ be a distribution on $\reals$, and consider its first moment $\expectedValue{\Q}{x}$. Now, via a simple Taylor expansion, we have that $\expectedValue{\Q}{f(x)}$ is a function of all the moments of $\Q$, and not just the first $p$ moments; see~\cite{jasour2021moment,kuehn2016moment} and references therein. 
Finally, a very common approach in practice is to approximate $\Q_0$ with some easy-to-handle parametrized probability distribution. However, even in this case, only few probability distributions (e.g., Gaussian distributions) are invariant even under linear dynamics, and their number decreases tremendously when the transformation is nonlinear.
\end{remark}
\end{comment}

\begin{corollary}[Deterministic dynamical systems] 
\label{cor:prop:nonlin:dyn}
Consider the dynamical system~\eqref{eq:nonlinear:dyn:sys}.
\begin{enumerate}
    \item If $f$ is invertible, then
    \begin{align*}
        x_t \sim \Q_t \in
        \ball{\varepsilon}{c_d \circ (f^{-t} \times f^{-t})}{\pushforward{f^{t}}\P},
    \end{align*}
    with $f^{t} = f \circ \ldots \circ f$ and $f^{-t} = f^{-1} \circ \ldots \circ f^{-1}$.
    
    \item If $f(x)=A x$ for $A \in \reals^{n\times n}$ and the transportation cost $c:\reals^n \to \nonnegativeReals$ is translation-invariant and orthomonotone, then
    \begin{align*}
        x_t \sim \Q_t \in \ball{\varepsilon}{c \circ \pinv{(A^t)}}{\pushforward{A^{t}} \P}.
    \end{align*}
\end{enumerate}
\end{corollary}

\begin{remark}[Norm bounded initial condition]
    \ldots 
\end{remark}

\begin{remark}[Distributonally Robust Monte Carlo]
The propagation of a probability distribution through a nonlinear map is itself a challenging task.
A common approach is to approximate $\Q_0$ with some easy-to-handle parametrized probability distribution. However, probability distributions are generally not invariant for a given dynamics, with one of the few exceptions being Gaussian distributions and linear dynamics. This makes the propagation inexact and errors difficult to quantify. 
\cref{cor:prop:nonlin:dyn} suggests an alternative method: One can propagate a \emph{finite} number of samples from $\Q_0$, which are available in most practical applications and use \cref{cor:prop:nonlin:dyn} to understand how the distributional uncertainty (introduced by the sampling and captured by the ambiguity set $\ball{\varepsilon}{c_d}{\empiricalP{n}}$) propagates through the dynamics.

\begin{comment}
However, in most applications, the distribution $\Q_0$ is generally unknown. Instead, it is very common to have some partial knowledge about $\Q_0$, such as some information about its first $p$ moments. Nonetheless, moments do not naturally propagate through the nonlinear dynamics. Indeed, let $\Q$ be a distribution on $\reals$, and consider its first moment $\expectedValue{\Q}{x}$. Now, via a simple Taylor expansion, we have that $\expectedValue{\Q}{f(x)}$ is a function of all the moments of $\Q$, and not just the first $p$ moments; see~\cite{jasour2021moment,kuehn2016moment} and references therein. 
Finally, 
A possible solution for the shortcomings presented in \cref{remark:shortcomingspropagation} is to propagate only a \emph{finite} number of samples from $\Q_0$, which are available in most practical applications. In that case, however, understanding how the distributional uncertainty (introduced by the sampling, and captured by the ambiguity set $\ball{\varepsilon}{c_d}{\empiricalP{n}}$) propagates through the dynamics becomes central. 
\end{comment}
\end{remark}

We now consider the setting of stochastic linear time-invariant control systems
\begin{align}
\label{eq:stoch:dyn:sys}
\begin{split}
    x_{t+1} &= A x_t + B u_t + D w_t\\
    u_t &= K x_t + v_t.
\end{split}
\end{align} 
where $u_t$ is the input, which consists of a feedback $Kx_t$ and a feedforward $v_t$, and $A \in \reals^{n \times n}$, $B \in \reals^{n \times m}$, $D \in \reals^{n \times r}$, and $K\in\reals^{m\times n}$. 
Differently from before, we now suppose that the initial condition $x_0 \in \reals^n$ is known and deterministic but the system dynamics are affected by process noise $w_t$, whose distribution is unknown.
Specifically, the noise sequence $\{w_t\}_{t\in\mathbb N} \subset \reals^r$ is i.i.d. according to an unknown light-tailed distribution $\P$ that belongs to the \gls{acr:ot} ambiguity set $\ball{\varepsilon}{\|\cdot\|_2^2}{\empiricalP{}}$, with reference distribution $\empiricalP{}$ and (translation-invariant and orthomonotone) transportation cost $c(\cdot) = \|\cdot\|_2^2$.

As above, we aim at quantifying the distributional uncertainty of the state $x_t$ at time $t$. 
For any $t\in\naturals$,  define the vectors $\mathbf{v}_{[t-1]} = \begin{bmatrix} v_{t-1}^\top & \cdots & v_0^\top \end{bmatrix}^\top$ and $\mathbf{w}_{[t-1]} = \begin{bmatrix}w_{t-1}^\top & \cdots & w_0^\top \end{bmatrix}^\top$. By linearity, the system dynamics~\eqref{eq:stoch:dyn:sys} can be rewritten as 
\begin{align}
\label{eq:stoch:dyn:sys:0-t}
\begin{split}
    x_{t} &= (A+BK)^t x_0 + \mathbf{B}_{t-1} \mathbf{v}_{[t-1]} + \mathbf{D}_{t-1} \mathbf{w}_{[t-1]}, \\
    \mathbf{B}_{t-1} &= \begin{bmatrix}B & (A+BK) B & \ldots & (A+BK)^{t-1} B \end{bmatrix}, \\ 
    \mathbf{D}_{t-1} &= \begin{bmatrix} D & (A+BK) D & \ldots & (A+BK)^{t-1} D \end{bmatrix}.
\end{split}
\end{align}
%\begin{assumption}
%\label{assump:D_t:fullrowrank}
%    The matrix $\mathbf{D}_{t-1}$ is full row-rank.
%\end{assumption}
%Assumption~\ref{assump:D_t:fullrowrank} trivially holds if $D$ is the identity matrix. Alternatively, the feedback gain matrix $K$ can be appropriately chosen to guarantee that this is satisfied.
Thus, the distributional uncertainty of the state $x_t$ results from the pushforward via the matrix $\mathbf{D}_{t-1}$ of the \gls{acr:ot} ambiguity set associated to $\mathbf{w}_{[t-1]}$.

\begin{proposition}
\label{prop:ambiguity:set:state}
Consider the linear control system~\eqref{eq:stoch:dyn:sys} and let $\ball{\varepsilon}{\|\cdot\|_2^2}{\empiricalP{}}$ capture the distributional uncertainty of $\{w_t\}_{t\in\naturals}$. Then, the distributional uncertainty of $x_t$ is captured by
\begin{align}
\label{eq:ambiguity:x_t}
    \ball{\varepsilon}{\|\cdot\|_2^2\circ \pinv{\mathbf{D}_{t-1}}}{\pushforward{((A+BK)^t x_0 + \mathbf{B}_{t-1} \mathbf{v}_{[t-1]}+\mathbf{D}_{t-1}x)}\empiricalP{}}.
\end{align}
Moreover, if $x_0\sim \mathbb{Q}$ and $\mathbf{D}_{t-1}$ is full row-rank, the the distributional uncertainty of $x_t$ is contained in
\begin{align}
\label{eq:ambiguity:x_t:x_0random}
    \ball{t \varepsilon}{\|\cdot\|_2^2\circ \pinv{\mathbf{D}_{t-1}}}{\pushforward{(A+BK)^t}\Q \ast \delta_{\mathbf{B}_{t-1} \mathbf{v}_{[t-1]}}\ast\pushforward{\mathbf{D}_{t-1}}{\empiricalP{}}}.
\end{align}
\end{proposition}
\begin{proof}
By~\cref{lemma:conc:ineq:noise}, the \gls{acr:ot} ambiguity set $\ball{t \varepsilon}{\|\cdot\|_2^2}{\empiricalP{}^{\otimes t}}$ captures the distributional uncertainty of the noise trajectory $\mathbf{w}_{[t-1]}$. Moreover, since the transportation cost $\|\cdot\|_2^2$ satisfies~\cref{assump:transportation:cost},~\cref{thm:lin:trans} establishes that the distributional uncertainty of the term $\mathbf{D}_{t-1} \mathbf{w}_{[t-1]}$ is captured by $\ball{t \varepsilon}{\|\cdot\|_2^2 \circ \pinv{\mathbf{D}_{t-1}}}{\pushforward{\mathbf{D}_{t-1}}{\empiricalP{}^{\otimes t}}}$. We now need to consider the sum with the deterministic term $(A+BK)^t x_0 + \mathbf{B}_{t-1} \mathbf{v}_{[t-1]}$. This is a simple translation, \cref{cor:lin:trans:specialcase} leads~\eqref{eq:ambiguity:x_t}.
If, instead, $x_0$ is not deterministic and distributed according to $\Q$, then~\cref{cor:known:noise} readily gives~\eqref{eq:ambiguity:x_t:x_0random}, provided that $\norm{\cdot}^2\circ\pinv{\mathbf{D}_{t-1}}$ is positive definite (i.e., $\mathbf{D}_{t-1}$ is full row-rank).  
This concludes the proof.
\end{proof}

We refer to the conference version of this paper for details on the ambiguity radius, the center, and the transportation cost. 


\subsection{Distributionally Robust Trajectory Planning}
\label{sec:application:trajectory:planning}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.9\linewidth]{cvar.pdf}
    \caption{CVaR is the expected value of the right $\delta$-tail.}
    \label{fig:cvar}
\end{figure}

We now instantiate our results for distributionally robust trajectory planning, whereby we aim at steering the system~\eqref{eq:stoch:dyn:sys} from a given initial condition to a target set. 
In particular, we seek the cheapest feedforward input sequence $\mathbf{v}_{[t-1]}$ steering the system~\eqref{eq:stoch:dyn:sys} from a deterministic initial condition $x_0$ to a given polyhedral set
\begin{equation}\label{eq:app:polyhedron}
    \mathcal X \coloneqq %\{x \in \reals^n:\, A x \leq b\}\\
    \left\{x \in \reals^n:\, \max_{j \in [J]} a_j^\top x + b_j \leq 0,\; J \in \mathbb N\right\},
\end{equation}
where $a_j\in\reals^n$ and $b_j\in\reals$.
To deal with distributions with unbounded support and reduce conservatism, we say an input trajectory $\mathbf{v}_{[t-1]}$ is feasible if the probability distribution of the state $x_t$ at time $t$, given by $\Q_t=\pushforward{((A+BK)^t x_0 + \mathbf{B}_{t-1} \mathbf{v}_{[t-1]}+\mathbf{D}_{t-1}x)}\empiricalP{}$, satisfies 
\begin{equation}\label{eq:app:CVaR:constraint}
    \text{CVaR}_{1-\gamma}^{\Q_t}\left(\max_{j \in [J]} a_j^\top x_t + b_j\right) \leq 0,
\end{equation} 
where, for a function $f:\reals^n \to \reals$ and a random variable $x\sim\Q$ on $\reals^n$, the CVaR of $f(x)$ at probability level $1-\gamma$ is
\begin{align}
\label{eq:CVaR}
    \text{CVaR}_{1-\gamma}^{\Q}(f(x))
    \coloneqq 
    \inf_{\tau \in \reals}\; \tau + \frac{1}{\gamma} \mathbb E_{\mathbb Q} \left[ \max\{0,f(x)-\tau\} \right].
\end{align}
The constraint $\text{CVaR}_{1-\gamma}^{\Q}(f(x))\leq 0$ is a convex relaxation of the more classical chance constraint  given by $\text{Pr}^{\Q}(f(x)\leq 0)\geq 1-\alpha$. Accordingly,~\eqref{eq:app:CVaR:constraint} can be interpreted as the convexification of probability that $x_t$ belongs to the target set $\mathcal{X}$ with probability of at least $1-\gamma$; see~\cref{fig:cvar}. 

If the true distribution $\Q_t$ of the state $x_t$ were known, the cheapest feedforward input results from
\begin{equation}\label{eq:dr trajectory}
\begin{array}{cl}
        \min & \displaystyle\sum_{t=0}^{t-1} \norm{v_t}_2^2 \\
        \st & \DS \text{CVaR}_{1-\gamma}^{\Q_t}\left(\max_{j \in [J]} a_j^\top x_t + b_j\right) \leq 0.
\end{array}
\end{equation}
We consider instead the case where the distribution is unknown and we only have access to $n$ i.i.d.\ noise samples $\{\widehat{w}^{(i)}\}_{i=1}^N$, yielding the $N$ noise sample trajectories 
\begin{align*}
    \widehat{\mathbf{w}}_{[t-1]}^{(i)}
    \coloneqq 
    \begin{bmatrix}(\widehat{w}_{t-1}^{(i)})^\top & \cdots & (\widehat{w}_0^{(i)})^\top \end{bmatrix}^\top,
\end{align*}
for $i \in \{1,\ldots,N\}$.
Under the assumption that the matrix $\mathbf{D}_{t-1}$ is full row-rank,~\cref{prop:ambiguity:set:state} gives the distributional uncertainty of $x_t$ is captured by
\begin{equation*}
\begin{aligned}
    \mathbb{S}_t&(\mathbf{v}_{[t-1]})\coloneqq
    \\
    &\ball{\varepsilon}{\|\cdot\|_2^2\circ \pinv{\mathbf{D}_{t-1}}}{\!\pushforward{((A+BK)^t x_0 + \mathbf{B}_{t-1} \mathbf{v}_{[t-1]}+\mathbf{D}_{t-1}x)}{\empiricalP{}^{}}}.
\end{aligned}
\end{equation*}
In particular, the center of the \gls*{acr:ot} ambiguity set $\mathbb{S}_t(\mathbf{v}_{[t-1]})$ is supported on the $N$ controlled state samples
\begin{align*}
    \widehat{x}_t^{(i)}(\mathbf{v}_{[t-1]})
    = (A+BK)^t x_0 + \mathbf{B}_{t-1} \mathbf{v}_{[t-1]} + \mathbf{D}_{t-1} \widehat{\mathbf{w}}_{[t-1]}^{(i)}.
\end{align*}
Accordingly, the optimal input results from the~\gls{acr:dro} problem, where the CVaR constraint~\eqref{eq:app:CVaR:constraint} must hold for all probability distribution belonging to $\mathbb{S}_t(\mathbf{v}_{[t-1]})$:
\begin{equation}\label{eq:dr trajectory}
\begin{array}{cl}
        \min & \displaystyle\sum_{t=0}^{t-1} \norm{v_t}_2^2 \\
        \st & \DS \sup_{\Q \in \mathbb{S}_t(\mathbf{v}_{[t-1]})} \text{CVaR}_{1-\gamma}^{\Q}\left(\max_{j \in [J]} a_j^\top x_t + b_j\right) \leq 0.
\end{array}
\end{equation}
With tools from~\gls{acr:dro}, \eqref{eq:dr trajectory} can be reformulated as a finite-dimensional convex optimization problem.  
\begin{proposition}
\label{prop:app:distributionally robust trajectory:reformulation}
The distributionally robust trajectory planning~\eqref{eq:dr trajectory} admits the finite-dimensional convex reformulation
\begin{align*}
    \begin{array}{cl}
        \min & \DS \|\mathbf{v}_{[t-1]}\|_2^2 \\
        \st 
        & \DS \lambda \varepsilon N + \sum_{i=1}^{N} s_{i} \leq 0
        \\
        & \DS
        \begin{aligned}[c]
        a_j^\top &\widehat{x}_t^{(i)}(\mathbf{v}_{[t-1]}) + b_j + \gamma \tau - \tau + \frac{1}{4\lambda\gamma} \\
        & a_j^\top \left((\pinv{\mathbf{D}_{t-1}})^\top \pinv{\mathbf{D}_{t-1}} \right)^{-1} a_j \leq \gamma s_i
        \end{aligned}
        \quad 
        \forall i \in [N], j\in [J]
        \\
        & \DS
        \tau\leq s_i \qquad  \forall i\in[N]
        \\
        & \DS 
        \tau \in \reals, \lambda \in \reals_+, s_i \in \reals.
    \end{array}
\end{align*}
\end{proposition}
The proof of this result follows readily from~\cite[Proposition 5]{aolaritei2023capture} and is therefore omitted.

We evaluate our methodology on the two-dimensional linear system $A=\frac{1}{2}\begin{bsmallmatrix} 1 & -1 \\ 2 & 1\end{bsmallmatrix}$, $B=I$, and $D=0.1 I$, with $K$ being the LQR controller (designed with $Q=R=I$) and $t=10$.
We suppose that the decision-maker has access to 5 noise sample trajectories. We choose the set $[1,2]\times [1,2]$ as the target (grey in~\cref{fig:trajectory:planning}) and select $\gamma=0.1$. We repeat our experiments for three values of $\varepsilon$ and compare with propagation of the \gls{acr:ot} ambiguity set via the Lipschitz constant and propagation of the center only.
As shown in \cref{fig:trajectory:planning}, the feedforward input resulting from $\varepsilon=0$ (red in~\cref{fig:trajectory:planning}) performs well on the 5 sample trajectories, steering them to the boundary of the target set, but yields poor performance on unseen samples. For larger $\varepsilon$ (blue and green in~\cref{fig:trajectory:planning}), instead, the system trajectories are successfully steered to the target set, even for unseen noise realizations, at the price of a slight increase in cost. Finally, the propagation via the Lipschitz constant yields instead 21\% larger cost, whereas only propagating the center leads to infeasibility. 

\begin{figure}[t]
    \centering
    \includegraphics[width=9cm,trim={0 1cm 0 2.8cm},clip]{figures/dr_steering.pdf}
    \caption{Distributionally robust steering of a system from the origin to a target set (in grey) for various radii $\varepsilon$. Filled circles (with solid lines) are the training samples and crosses (with dotted lines) are testing samples. Small radii lead to trajectories approaching the boundary of the target, which however might not reach the target under different noise realizations (in red); larger radii, instead, push the trajectory to the interior of the target (in green).}
    \label{fig:trajectory:planning}
    \vspace{-.3cm}
\end{figure}


\subsection{Consensus in Averaging Algorithms}
\label{sec:application:consensus}
We now study the uncertainty quantification of the consensus state of an averaging algorithm. Consider the discrete-time averaging algorithm with random initial condition
\begin{equation*}
    x_{t+1}=Ax_t\qquad x_0\sim\P_0\in\probSpace{\reals^n},
\end{equation*}
where $A\in\reals^{n\times n}$ is the (row-stochastic) adjacency matrix associated with a directed graph $G$ (which captures the interactions among the nodes/agents of the averaging).
Such algorithms are ubiquitous in many applications, including network systems, multi-agent systems, and opinion dynamics; e.g., see~\cite{garin2010survey,bullo2020lectures} and references therein. 

In many-real world settings, the probability distribution of the initial condition $\P_0$ is unknown. Accordingly, we can use an \gls*{acr:ot} ambiguity set $\ball{\varepsilon}{c}{\empiricalP{0}}$ to capture its distributional uncertainty. 
For instance, in opinion dynamics, the distribution of users' initial opinions is unknown but can be estimated via surveys; in sensor networks, $\empiricalP{0}$ can be calibrated based on the sensors' specifications.
Here, we are interested in capturing the distributional uncertainty of the consensus state $\lim_{t\to\infty}x_t$.

\begin{proposition}\label{prop:app:consensus}
Suppose that either (i) the directed graph $G$ has a globally reachable node and the subgraph of globally reachable nodes is aperiodic or, equivalently, (ii) $A$ has a unique eigenvalue in $1$ and all the others are strictly inside the unit circle.
Let $x_t\sim\P_t$ the probability distribution associated with the state $x_t$ and $h:\reals^n\to\reals^n$ defined as $h(x)=(\T{w} x) \ones_n$ with $w$ being the left eigenvector of $A$ corresponding to the eigenvalue $1$ (normalized so that $\T \ones_n w =1$). Then,
\begin{align*}
    \P_t \to \pushforward{h} \P_0 \in \pushforward{(\ones_n)} \ball{\varepsilon}{c \circ w}{\pushforward{\T{w}} \empiricalP{0}}.
    %\subset \otimes_{i=1}^d \mathbb B_{|\entry{v}{i}|^p\varepsilon}^{c \circ \pinv{w}}(\pushforward{w} \P)
\end{align*} 
If additionally $c$ is homogeneous of degree $p$
\begin{align*}
    \P_t \to \pushforward{h} \P_0 \in \pushforward{(\ones_n)} \ball{\varepsilon/c(w)}{\abs{\cdot}^p}{\pushforward{\T{w}} \empiricalP{0}},
    %\subset \otimes_{i=1}^d \mathbb B_{|\entry{v}{i}|^p\varepsilon}^{c \circ \pinv{w}}(\pushforward{w} \P)
\end{align*}
If additionally $A$ is doubly-stochastic, then $w=\frac{1}{n}\ones_n$ and
\begin{align*}
    \P_t \to \pushforward{h} \P_0 \in \pushforward{(\ones_n)} \ball{\varepsilon d^p/c(\ones_n)}{\abs{\cdot}^p}{\pushforward{\textstyle{\frac{1}{n}}\T{\ones_n}} \empiricalP{0}}.
    %\subset \otimes_{i=1}^d \mathbb B_{|\entry{v}{i}|^p\varepsilon}^{c \circ \pinv{w}}(\pushforward{w} \P)
\end{align*}
%In particular, when $c$ is additionally homogeneous of degree $p$, 
%\begin{align*}
%    \pushforward{{\pi_i}} \Q_t \to \pushforward{{\pi_i}} \pushforward{h} \Q_0 \in \ball{\varepsilon}{c \circ w}{\pushforward{\T{w}}\P},
%    %\subset \otimes_{i=1}^d \mathbb B_{|\entry{v}{i}|^p\varepsilon}^{c \circ \pinv{w}}(\pushforward{w} \P)
%\end{align*}
%for all $i=1,\ldots,d$.
\end{proposition}

\begin{proof}
We first claim that $\Q_t \to \Q_\infty := \pushforward{h} \Q_0$, with $h$ as in the statement. If this is true, $\Q_\infty \in \pushforward{h} \ball{\varepsilon}{c}{\P}$, and the result follows from \cref{thm:lin:trans}. First, the transformation $x \mapsto \T{w} x$ is surjective. Therefore,~\eqref{eq:B_epsilon:surjective:A:1} implies that
\begin{align*}
    \pushforward{\T{w}} \ball{\varepsilon}{c}{\P} = \ball{\varepsilon}{c \circ \pinv{(\T w)}}{\pushforward{\T{w}} \P},
\end{align*}
with $\pinv{(\T w)} = w(\T{w} w)^{-1}$ being the right inverse of $\T w$. Since $w$ is normalized, we have that $\T w w = 1$, and thus $\pinv{(\T w)}  = w$. Notice that $\ball{\varepsilon}{c \circ w}{\pushforward{\T w} \P}$ is an ambiguity set of probability distributions over $\reals$. Then, $\pushforward{h} \Q_0 = \pushforward{\ones_n}\ball{\varepsilon}{c \circ w}{\pushforward{\T{w}} \P}$. %In particular, by~\cref{cor:lin:trans:specialcase}, we have that $\pushforward{{\pi_i}} \pushforward{h}\Q_0 = \ball{\varepsilon}{c \circ w}{\pushforward{\T{w}} \P} = \ball{\varepsilon}{c \circ w}{\pushforward{\T{w}} \P}$, whenever $c$ is homogeneous of degree $p$.
We now prove $\Q_t \to \pushforward{h} \Q_0$. First, from a standard modal decomposition of the matrix $A$, we have that $\Phi_t(x) = A^t x \to h(x) = (\T{w} x) v$ for all $x\in\reals^n$. Then, for any continuous and bounded test function $\phi: \reals^n \to \reals$,
\begin{align*}
    \int_{\reals^n} \phi(x) &\d\Q_t(x) 
    = 
    \int_{\reals^n} \phi(\Phi_t(x)) \d\Q_0(x)
    \\
    &\to
    \int_{\reals^n} \phi(h(x)) \d\Q_0(x)
    =
    \int_{\reals^n} \phi(x) \d(\pushforward{h}\Q_0)(x).
\end{align*}
If additionally $c$ is homogeneous of degree $p$, we have
\begin{equation*}
(c\circ w)(x-y)=c(wx-wy)=c(w(x-y))=\abs{x-y}^p c(w).
\end{equation*}
Since $c(w)$ is a constant, the statement readily follows from the definition of \gls{acr:ot} ambiguity set. If additionally $w=\frac{1}{n}\ones_n$, $c(w)=\frac{1}{n^p}c(\ones_n)$. This concludes the proof. 
\end{proof}

In words, the distributional uncertainty is the same on all entries of $\lim_{t\to\infty} x_t$ and it belongs to the \gls*{acr:ot} ambiguity set $\ball{\varepsilon}{c \circ w}{\pushforward{\T{w}} \empiricalP{0}}$, which therefore captures the distributional uncertainty of the consensus state. This way, for instance, we can quantify the worst-case probability that the consensus state resides outside of an interval $(a,b)$ of interest via
\begin{equation*}
    \sup_{\Q \in \ball{\varepsilon/c(w)}{\abs{\cdot}^p}{\pushforward{\T{w}} \empiricalP{0}}} \mathrm{Pr}(x\notin (a,b))=\int_{\reals\setminus(a,b)} \d\Q(x).
\end{equation*}
As above, this optimization problem admits a finite-dimensional convex reformulation.

%\subsection{Nonlinear Systems}
%\label{subsec:application:nonlinear}
%\ldots 
%\end{comment}


\subsection{Least Squares Estimation}\label{sec:LS}

Our last application concerns statistical estimation. Consider the linear inverse problem
\begin{align}
\label{eq:least:squares}
    y = A x_0 + z,
\end{align}
where the aim is to estimate the parameter $x_0 \in \reals^n$ from $m$ noisy measurements (with $m>n$) of the form $\entry{y}{i} = \T{a_i} x_0 + z_i$, where $z_i$ is random measurement noise and the $z_i$ are i.i.d. and distributed according to $\P_z$. If $A$ has full column-rank, a ubiquitous solution is the \gls{acr:ols} estimator
\begin{align}
\label{eq:least:squares:estimator}
    \hat{x}\coloneqq \argmin_{x \in \reals^n}\; \|y-Ax\|_2=\pinv{A} y = (\T A A)^{-1}\T A y.
\end{align}
It is well-known that the \gls{acr:ols} estimator corresponds to the maximum likelihood estimation when the measurement noise $\{(z_i)\}_{i=1}^m$ are standard normal with equal variances. Moreover, by the Gauss–Markov theorem \cite{sullivan2015introduction}, if $\{(z_i)\}_{i=1}^m$ have zero mean and equal finite variance, then the \gls{acr:ols} estimator is the best linear unbiased estimator, i.e., it has the lowest sampling variance within the class of linear unbiased estimators. 

Here, we depart from these assumptions and study a more general case, where we only have access to the $n$ i.i.d. samples $\{(\sample{z}{i})\}_{i=1}^n$ from an otherwise unknown measurement noise distribution $\P_z$. In this scenario, we seek to understand how the distributional uncertainty of measurement noise, captured by an \gls{acr:ot} ambiguity set, propagates to the \gls{acr:ols} estimator $\hat{x}$ in~\eqref{eq:least:squares:estimator}. 
In other words, we construct an \gls*{acr:ot} ambiguity set $\ball{\varepsilon}{c}{\empiricalP{z,N}}$ centered at the empirical distribution $\empiricalP{z,N} = n^{-1}\sum_{i=1}^n \delta_{\sample{z}{i}}$, which is guaranteed to contain the true probability distribution $\P_z$ with high probability and study the resulting \gls*{acr:ot} ambiguity set around the estimation error $\hat{x} - x_0$.
Especially when the \gls{acr:ols} estimator is subsequently used for decision-making (e.g., in estimation problems), it is crucial to dispose of an accurate quantification of the related uncertainty. 

Before proceeding to the main result of this section, we need a preparatory lemma. The lemma states that when an $m$-dimensional distribution is the $m$-fold product of some one-dimensional distribution, then the exponential dependence on the dimension in the concentration inequality in~\cite[Theorem 2]{Fournier2015} can be replaced by a linear dependence on the dimension. This will be crucial when constructing the ambiguity set around $\hat{x} - x_0$.

\begin{lemma}
\label{lemma:ols:conc:ineq:noise}
Let $Z$ be a one-dimensional random variable distributed according to $\P_z$, and let $\empiricalP{z,N} = \frac{1}{N} \sum_{i=1}^N \delta_{\sample{z}{i}}$ be the empirical distribution constructed using the $N$ i.i.d. samples $\{(\sample{z}{i})\}_{i=1}^N$. Moreover, let $\P_z^{\otimes m}$ and $\hat{\P}_{z,N}^{\otimes m}$ denote the $m$-fold product of $\P_z$ and $\hat{\P}_{z,N}$, respectively. Finally, let $c:\reals^m \to \nonnegativeReals$ be a translation-invariant transportation cost satisfying
\begin{align}
\label{lemma:conc:ineq:noise:assump:cost}
    c(x-y) \leq
    \sum_{i=1}^m (c \circ \pinv{\pi}_i)(\entry{x}{i}-\entry{y}{i})
    = \sum_{i=1}^m c((\entry{x}{i}-\entry{y}{i})\entry{e}{i}),
\end{align}
with $\{(\entry{e}{i})\}_{i=1}^m$ the standard basis in $\reals^m$. Then, the following two implications hold:
\begin{align}
\label{eq:lemma:conc:ineq:noise:1}
    \P_z^{\otimes m} \in \ball{\varepsilon}{c}{\empiricalP{z,N}^{\otimes m}}
    &\implies
    \P_z \in \ball{\varepsilon}{c \circ \pinv{\pi}_i}{\empiricalP{z,N}}\:\forall i\in [m]
\end{align}
and
\begin{align}
    \label{eq:lemma:conc:ineq:noise:2}
    \P_z \in \ball{\varepsilon_i}{c \circ \pinv{\pi}_i}{\empiricalP{z,N}}
    \; \forall i \in [m]
    &\implies
    \P_z^{\otimes m} \in \ball{\varepsilon_1 + \ldots + \varepsilon_m}{c}{\empiricalP{z,N}^{\otimes m}}.
\end{align}
\end{lemma}

\begin{proof}
We start by proving the first implication \eqref{eq:lemma:conc:ineq:noise:1}. Notice first that $\pushforward{{\pi_i}} \P_z^{\otimes m} = \P_z$ and $\pushforward{{\pi_i}} \empiricalP{z,N}^{\otimes m} = \empiricalP{z,N}$. Moreover, from \cref{eq:B_epsilon:surjective:A:1} in~\cref{thm:lin:trans}, we have that
\begin{align*}
    \P_z = \pushforward{{\pi_i}} \P_z^{\otimes m} 
    \in 
    \pushforward{{\pi_i}} \ball{\varepsilon}{c}{\empiricalP{z,N}^{\otimes m}}
    &=
    \ball{\varepsilon}{c \circ \pinv{\pi}_i}{\pushforward{{\pi_i}}\empiricalP{z,N}^{\otimes m}}
    \\
    &=
    \ball{\varepsilon}{c \circ \pinv{\pi}_i}{\empiricalP{z,N}},
\end{align*}
concluding the proof of \eqref{eq:lemma:conc:ineq:noise:1}.

We will now prove the second implication~\eqref{eq:lemma:conc:ineq:noise:2}. Let $\gamma_i \in \setPlans{\P_z}{\empiricalP{z,N}}$ be the optimal coupling associated to the transportation cost $c \circ \pinv{\pi}_i:\reals\to\nonnegativeReals$, and satisfying
\begin{align*}
    \int_{\reals \times \reals} (c \circ \pinv{\pi}_i)(x_i-y_i) \d\gamma_i(x_i,y_i) 
    \leq 
    \varepsilon_i.
\end{align*}
It is easy to see that the product distribution $\otimes_{i=1}^m \gamma_i$ belongs to the set of coupling $\setPlans{\P_z^{\otimes m}}{\empiricalP{z,N}^{\otimes m}}$. Then, we have that 
\begin{align*}
    &\hspace{-0.8cm}\inf_{\gamma \in \setPlans{\P_z^{\otimes m}}{\empiricalP{z,N}^{\otimes m}}} \int_{\reals^m \times \reals^m} c (x-y) \d\gamma(x,y) 
    \\
    &\leq 
    \int_{\reals^m \times \reals^m} c (x-y) \d(\otimes_{i=1}^m \gamma_i)(x,y)
    \\ &\leq
    \int_{\reals^m \times \reals^m} \sum_{i=1}^m (c \circ \pinv{\pi}_i)(\entry{x}{i}-\entry{y}{i}) \d(\otimes_{i=1}^m \gamma_i)(x,y)
    \\ &=
    \sum_{i=1}^m\int_{\reals \times \reals} (c \circ \pinv{\pi}_i)(\entry{x}{i}-\entry{y}{i}) \d\gamma_i(\entry{x}{i},\entry{y}{i})
    \\ &\leq
    \varepsilon_1 + \ldots + \varepsilon_m,
\end{align*}
from which we can conclude that $\P_z^{\otimes m} \in \ball{\varepsilon_1 + \ldots + \varepsilon_m}{c}{\empiricalP{z,N}^{\otimes m}}$.
\end{proof}


\begin{remark}
Practically, this result can be used as follows. First, the concentration inequality from~\cite[Theorem 2]{Fournier2015} can be employed to find the radii $\varepsilon_i$ which guarantee that $ \P_z \in \ball{\varepsilon_i}{c \circ \pinv{\pi}_i}{\empiricalP{z,N}}$, for all $i\in[m]$. Notice that this can be done efficiently (in the number of samples $\{(\sample{z}{i})\}_{i=1}^N$) since the underlying space is one-dimensional. Subsequently, the second implication of~\eqref{lemma:conc:ineq:noise:assump:cost} is employed to construct an ambiguity set in $m$ dimensions (with $m$ possibly very large), without suffering from the curse of dimensionality appearing in the concentration inequality of~\cite[Theorem 2]{Fournier2015}.
\end{remark}

Armed with~\cref{lemma:conc:ineq:noise,thm:lin:trans}, we are now ready to quantify the distributional uncertainty of the~\gls{acr:ols} estimator.

\begin{proposition}[Distributional uncertainty of \gls{acr:ols} estimator]
\label{prop:leastsquares}
Consider the linear inverse problem \eqref{eq:least:squares}, with $y \in \reals^m$, $x_0 \in \reals^n$ (deterministic or random), and $m>n$, where the (known) matrix $A$ is full column-rank, and $z = \T{(z_1,\ldots,z_m)}$ is the measurement noise vector distributed according to $\P_z^{\otimes m}$. Moreover, let $\empiricalP{z,N} = \frac{1}{N} \sum_{i=1}^N \delta_{\sample{z}{i}}$ be the empirical distribution constructed using $N$ i.i.d. samples $\{(\sample{z}{i})\}_{i=1}^N$, and let $\varepsilon_i$ be such that $\P_z \in \ball{\varepsilon_i}{c \circ \pinv{\pi}_i}{\empiricalP{z,N}}$, for all $i \in \{1,\ldots,m\}$, for a translation-invariant and orthomonotone transportation cost $c$ satisfying \eqref{lemma:conc:ineq:noise:assump:cost}. Finally, let $\hat{x}$ denote the \gls{acr:ols} estimator of $x_0$, defined in \eqref{eq:least:squares:estimator}. Then, we have that
\begin{align}
\label{eq:prop:leastsquares}
    \hat{x} - x_0 \sim \Q \in \ball{\varepsilon_1 + \ldots + \varepsilon_m}{c \circ A}{\pushforward{\pinv{A}} \empiricalP{z,N}^{\otimes m}},
\end{align}
i.e., the distribution of $\hat{x} - x_0$ is contained in the ambiguity set $\ball{\varepsilon_1 + \ldots + \varepsilon_m}{c \circ A}{\pushforward{\pinv{A}} \empiricalP{z,N}^{\otimes m}}$.
\end{proposition}
\begin{proof}
By~\eqref{eq:least:squares:estimator}, $\hat{x} = \pinv{A} y = \pinv{A} (A x_0 + z) = x_0 + \pinv{A} z$ or, equivalently, $\hat{x} - x_0 = \pinv{A} z$, with $\pinv{A} = \inv{(\T A A)}\T A$ being the left inverse of $A$. Therefore, $\hat{x} - x_0$ is distributed as $\pinv{A} z$, i.e., $\Q = \pushforward{\pinv{A}}\P_z^{\otimes m}$. Now, using Lemma~\ref{lemma:conc:ineq:noise} and the assumption that $\P_z \in \ball{\varepsilon_i}{c \circ \pinv{\pi}_i}{\empiricalP{z,N}}$, for all $i \in \{1,\ldots,m\}$, we have that $\P_z^{\otimes m} \in \ball{\varepsilon_1 + \ldots + \varepsilon_m}{c}{\empiricalP{z,N}^{\otimes m}}$. Finally, since $A$ has full column-rank, we have that $\pinv{A}$ has full row-rank, and therefore we can use the equality \eqref{eq:B_epsilon:surjective:A:1} from~\cref{thm:lin:trans} and get
\begin{align*}
    \Q
    =
    \pushforward{\pinv{A}} \P_z^{\otimes m} 
    &\in \pushforward{\pinv{A}} \ball{\varepsilon_1 + \ldots + \varepsilon_m}{c}{\empiricalP{z,N}^{\otimes m}}
    \\
    &=
    \ball{\varepsilon_1 + \ldots + \varepsilon_m}{c \circ A}{\pushforward{\pinv{A}} \empiricalP{z,N}^{\otimes m}},
\end{align*}
since $A$ is the right inverse of $\pinv{A}$. This concludes the proof.
\end{proof}

\begin{remark}
When the measurement noise has zero mean and variance $\sigma^2_z$, the covariance matrix of the \gls{acr:ols} estimator is equal to $\inv{(\T{A}A)}\sigma_z^2$ \cite{sullivan2015introduction}.
However, except for basic cases (e.g., Gaussian measurement noise), the covariance will not entirely capture the distributional uncertainty of the \gls{acr:ols} estimator. On the contrary, \cref{prop:leastsquares} enables us to fully capture the distributional uncertainty of estimation error $\hat{x}  - x_0$.

==> old/dynamical_old.tex <==

\newpage 
.
\newpage
.
\newpage
.
\newpage

\subsection{Dynamical Systems and Control Theory}\label{sec:app:dynamical}
Our first application concerns the propagation of the distributional uncertainty through a dynamical system. To start, consider the deterministic dynamical system
\begin{align}
    x_{t+1} = f(x_t), \quad x_0 \sim \Q_0 \in \ball{\varepsilon}{c}{\P},
\end{align}
with $f:\reals^n \to \reals^n$. %The notation $x^+$ stands for either discrete-time, in which case \eqref{eq:nonlinear:dyn:sys} is a difference equation, i.e. $x_{t+1} = f(x_t)$, or continuous-time, in which case \eqref{eq:nonlinear:dyn:sys} is an ordinary differential equation, i.e. $\dot{x} = f(x)$. 
%We denote by $\Phi_t(x_0)$ the solution map of the dynamical system \eqref{eq:nonlinear:dyn:sys} at time $t$, parametrized by the initial condition $x_0$.
%Later in this section, we will also consider the case of stochastic dynamical systems.
The initial condition $x_0$ is distributed according to some unknown probability distribution $\Q_0$, which is however known to belong to the ambiguity set $\ball{\varepsilon}{c_d}{\P}$ with center $\P\in\probSpace{\reals^d}$. This formulation encompasses the scenario when one only has access to $n$ i.i.d. samples $\{(\sample{x_0}{i})\}_{i=1}^n$ from $\Q_0$. In this case, the concentration inequality of~\cref{prop:conc:ineq} can be used to construct an \gls{acr:ot} ambiguity set $\ball{\varepsilon}{c}{\empiricalP{n}}$ around the empirical distribution $\empiricalP{n} = \frac{1}{n}\sum_{i=1}^n \diracDelta{\sample{x_0}{i}}$ which contains the true distribution $\P$ with high probability.

We now study how the distributional uncertainty encapsulated in the \gls{acr:ot} ambiguity set $\ball{\varepsilon}{c_d}{\P}$ propagates through the dynamics. This way, we can characterize the distributional uncertainty of $x_t$, which enables, among others, distributionally robust analysis and decision-making; see~\cref{sec:application:trajectory:planning} on distributionally robust trajectory planning below for an example. 
Since~\eqref{eq:nonlinear:dyn:sys} is effectively a pushforward via $f\circ\ldots\circ f$ of $\Q_0$, the result follows directly from~\cref{thm:nonlin:trans,thm:lin:trans}:

\begin{comment}
\begin{remark}\label{remark:shortcomingspropagation}
Whenever the initial distribution $\Q_0$ is known and absolutely continuous with density $\rho_0$, i.e. $\Q_0=\rho_0\lebesgueMeasure{d}$, and the transformation $f$ is a diffeomorphism,~\eqref{eq:propagation:abs:cont:distrib} can be used to recover the distribution of $\Phi_t(x_0)$ as
\begin{align*}
    \Phi_t(x_0) \sim \Q_t = \frac{\rho\circ f^{-t}}{|\det\nabla (f^t)|}\lebesgueMeasure{d}.
\end{align*}
However, in most applications, the distribution $\Q_0$ is generally unknown. Instead, it is very common to have some partial knowledge about $\Q_0$, such as some information about its first $p$ moments. Nonetheless, moments do not naturally propagate through the nonlinear dynamics. Indeed, let $\Q$ be a distribution on $\reals$, and consider its first moment $\expectedValue{\Q}{x}$. Now, via a simple Taylor expansion, we have that $\expectedValue{\Q}{f(x)}$ is a function of all the moments of $\Q$, and not just the first $p$ moments; see~\cite{jasour2021moment,kuehn2016moment} and references therein. 
Finally, a very common approach in practice is to approximate $\Q_0$ with some easy-to-handle parametrized probability distribution. However, even in this case, only few probability distributions (e.g., Gaussian distributions) are invariant even under linear dynamics, and their number decreases tremendously when the transformation is nonlinear.
\end{remark}
\end{comment}

\begin{corollary}[Deterministic dynamical systems] 
\label{cor:prop:nonlin:dyn}
Consider the dynamical system~\eqref{eq:nonlinear:dyn:sys}.
\begin{enumerate}
    \item If $f$ is invertible, then
    \begin{align*}
        x_t \sim \Q_t \in
        \ball{\varepsilon}{c_d \circ (f^{-t} \times f^{-t})}{\pushforward{f^{t}}\P},
    \end{align*}
    with $f^{t} = f \circ \ldots \circ f$ and $f^{-t} = f^{-1} \circ \ldots \circ f^{-1}$.
    
    \item If $f(x)=A x$ for $A \in \reals^{n\times n}$ and the transportation cost $c:\reals^n \to \nonnegativeReals$ is translation-invariant and orthomonotone, then
    \begin{align*}
        x_t \sim \Q_t \in \ball{\varepsilon}{c \circ \pinv{(A^t)}}{\pushforward{A^{t}} \P}.
    \end{align*}
\end{enumerate}
\end{corollary}

\begin{remark}[Norm bounded initial condition]
    \ldots 
\end{remark}



We now consider the setting of stochastic linear time-invariant control systems
\begin{align}
\label{eq:stoch:dyn:sys}
\begin{split}
    x_{t+1} &= A x_t + B u_t + D w_t\\
    u_t &= K x_t + v_t.
\end{split}
\end{align} 
where $u_t$ is the input, which consists of a feedback $Kx_t$ and a feedforward $v_t$, and $A \in \reals^{n \times n}$, $B \in \reals^{n \times m}$, $D \in \reals^{n \times r}$, and $K\in\reals^{m\times n}$. 
Differently from before, we now suppose that the initial condition $x_0 \in \reals^n$ is known and deterministic but the system dynamics are affected by process noise $w_t$, whose distribution is unknown.
Specifically, the noise sequence $\{w_t\}_{t\in\mathbb N} \subset \reals^r$ is i.i.d. according to an unknown light-tailed distribution $\P$ that belongs to the \gls{acr:ot} ambiguity set $\ball{\varepsilon}{\|\cdot\|_2^2}{\empiricalP{}}$, with reference distribution $\empiricalP{}$ and (translation-invariant and orthomonotone) transportation cost $c(\cdot) = \|\cdot\|_2^2$.

As above, we aim at quantifying the distributional uncertainty of the state $x_t$ at time $t$. 
For any $t\in\naturals$,  define the vectors $\mathbf{v}_{[t-1]} = \begin{bmatrix} v_{t-1}^\top & \cdots & v_0^\top \end{bmatrix}^\top$ and $\mathbf{w}_{[t-1]} = \begin{bmatrix}w_{t-1}^\top & \cdots & w_0^\top \end{bmatrix}^\top$. By linearity, the system dynamics~\eqref{eq:stoch:dyn:sys} can be rewritten as 
\begin{align}
\label{eq:stoch:dyn:sys:0-t}
\begin{split}
    x_{t} &= (A+BK)^t x_0 + \mathbf{B}_{t-1} \mathbf{v}_{[t-1]} + \mathbf{D}_{t-1} \mathbf{w}_{[t-1]}, \\
    \mathbf{B}_{t-1} &= \begin{bmatrix}B & (A+BK) B & \ldots & (A+BK)^{t-1} B \end{bmatrix}, \\ 
    \mathbf{D}_{t-1} &= \begin{bmatrix} D & (A+BK) D & \ldots & (A+BK)^{t-1} D \end{bmatrix}.
\end{split}
\end{align}
%\begin{assumption}
%\label{assump:D_t:fullrowrank}
%    The matrix $\mathbf{D}_{t-1}$ is full row-rank.
%\end{assumption}
%Assumption~\ref{assump:D_t:fullrowrank} trivially holds if $D$ is the identity matrix. Alternatively, the feedback gain matrix $K$ can be appropriately chosen to guarantee that this is satisfied.
Thus, the distributional uncertainty of the state $x_t$ results from the pushforward via the matrix $\mathbf{D}_{t-1}$ of the \gls{acr:ot} ambiguity set associated to $\mathbf{w}_{[t-1]}$.

\begin{proposition}
\label{prop:ambiguity:set:state}
Consider the linear control system~\eqref{eq:stoch:dyn:sys} and let $\ball{\varepsilon}{\|\cdot\|_2^2}{\empiricalP{}}$ capture the distributional uncertainty of $\{w_t\}_{t\in\naturals}$. Then, the distributional uncertainty of $x_t$ is captured by
\begin{align}
\label{eq:ambiguity:x_t}
    \ball{\varepsilon}{\|\cdot\|_2^2\circ \pinv{\mathbf{D}_{t-1}}}{\pushforward{((A+BK)^t x_0 + \mathbf{B}_{t-1} \mathbf{v}_{[t-1]}+\mathbf{D}_{t-1}x)}\empiricalP{}}.
\end{align}
Moreover, if $x_0\sim \mathbb{Q}$ and $\mathbf{D}_{t-1}$ is full row-rank, the the distributional uncertainty of $x_t$ is contained in
\begin{align}
\label{eq:ambiguity:x_t:x_0random}
    \ball{t \varepsilon}{\|\cdot\|_2^2\circ \pinv{\mathbf{D}_{t-1}}}{\pushforward{(A+BK)^t}\Q \ast \delta_{\mathbf{B}_{t-1} \mathbf{v}_{[t-1]}}\ast\pushforward{\mathbf{D}_{t-1}}{\empiricalP{}}}.
\end{align}
\end{proposition}
\begin{proof}
By~\cref{lemma:conc:ineq:noise}, the \gls{acr:ot} ambiguity set $\ball{t \varepsilon}{\|\cdot\|_2^2}{\empiricalP{}^{\otimes t}}$ captures the distributional uncertainty of the noise trajectory $\mathbf{w}_{[t-1]}$. Moreover, since the transportation cost $\|\cdot\|_2^2$ satisfies~\cref{assump:transportation:cost},~\cref{thm:lin:trans} establishes that the distributional uncertainty of the term $\mathbf{D}_{t-1} \mathbf{w}_{[t-1]}$ is captured by $\ball{t \varepsilon}{\|\cdot\|_2^2 \circ \pinv{\mathbf{D}_{t-1}}}{\pushforward{\mathbf{D}_{t-1}}{\empiricalP{}^{\otimes t}}}$. We now need to consider the sum with the deterministic term $(A+BK)^t x_0 + \mathbf{B}_{t-1} \mathbf{v}_{[t-1]}$. This is a simple translation, \cref{cor:lin:trans:specialcase} leads~\eqref{eq:ambiguity:x_t}.
If, instead, $x_0$ is not deterministic and distributed according to $\Q$, then~\cref{cor:known:noise} readily gives~\eqref{eq:ambiguity:x_t:x_0random}, provided that $\norm{\cdot}^2\circ\pinv{\mathbf{D}_{t-1}}$ is positive definite (i.e., $\mathbf{D}_{t-1}$ is full row-rank).  
This concludes the proof.
\end{proof}

We refer to the conference version of this paper for details on the ambiguity radius, the center, and the transportation cost. 


